A Survey on Arabic Named Entity Recognition: Past, Recent Advances, and Future Trends

As more and more Arabic texts emerged on the Internet, extracting important information from these Arabic texts is especially useful. As a fundamental technology, Named entity recognition (NER) serves as the core component in information extraction technology, while also playing a critical role in many other Natural Language Processing (NLP) systems, such as question answering and knowledge graph building. In this paper, we provide a comprehensive review of the development of Arabic NER, especially the recent advances in deep learning and pre-trained language model. Specifically, we first introduce the background of Arabic NER, including the characteristics of Arabic and existing resources for Arabic NER. Then, we systematically review the development of Arabic NER methods. Traditional Arabic NER systems focus on feature engineering and designing domain-specific rules. In recent years, deep learning methods achieve significant progress by representing texts via continuous vector representations. With the growth of pre-trained language model, Arabic NER yields better performance. Finally, we conclude the method gap between Arabic NER and NER methods from other languages, which helps outline future directions for Arabic NER.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> background.tex <==
\subsection{What is Arabic NER}

\begin{table*}[t]
	\centering
	\caption{List of annotated datasets for Arabic NER. ``\#Tags'' refers to the number of entity types.}	
	\label{tab:datasets}
	\begin{tabular}{ccccp{8.2cm}}
		\toprule
		Corpus & Year & Text Source & \#Tags & URL \\ \midrule
		
    ANERcorp & 2007     &  Website, news, magazines           & 4       & \url{https://camel.abudhabi.nyu.edu/anercorp/}    \\
    ACE 2003 &  2004    &  	Broadcast News, newswire genres     & 7       & \url{https://catalog.ldc.upenn.edu/LDC2004T09} \\

    ACE 2004 &  2004    &  Broadcast News, newswire genres             & 7       & \url{https://catalog.ldc.upenn.edu/LDC2005T09} \\

    ACE 2005 &  2005    &  Transcripts,  news            & 7       & \url{https://catalog.ldc.upenn.edu/LDC2006T06} \\

    ACE 2007 &  2007    &  Transcripts,  news            & 7       & \url{https://catalog.ldc.upenn.edu/LDC2014T18} \\

    REFLEX &  2009    &  Reuters  news           & 4       & \url{https://catalog.ldc.upenn.edu/LDC2009T11}    \\

    AQMAR &  2012    &  Arabic Wikipedia            & 7       &   \url{http://www.cs.cmu.edu/~ark/ArabicNER/}  \\

    OntoNotes 5.0 &  2013    &  News            & 18       & \url{https://catalog.ldc.upenn.edu/LDC2013T19}    \\

    WDC &  2014    &  Wikipedia          &  4       & \url{https://github.com/Maha-J-Althobaiti/Arabic_NER_Wiki-Corpus}    \\

    DAWT & 2017    &  Wikipedia           & 4    & \url{https://github.com/klout/opendata/tree/master/wiki_annotation}    \\

    % NE3L &   1997  &     New York Times news         &   7     &    \url{http://catalog.elra.info/en-us/repository/browse/ELRA-W0078/}  \\
    CANERCorpus & 2018  & Religion  & 20 & https://github.com/RamziSalah/Classical-Arabic-Named-Entity-Recognition-Corpus
    \\      

    Wojood &  2022    &  Wikipedia        & 21     & \url{https://ontology.birzeit.edu/Wojood/}    \\


			 \bottomrule
	\end{tabular}
\end{table*}


Arabic NER aims to locate and classify named entities in Arabic text $s=<w_n, ..., w_2, w_1>$ (Different from the left-to-right style of writing in Chinese or English, Arabic is writing from right to left) into predefined entity categories. Same as other common NER tasks, the Arabic NER can also be divided into general domain including Person, Location and Organization types, and specific domain (e.g. Biomedical, News and Finance).

There are two typical outputs for NER, one is a list of tuples $<P_s, P_e, t>$, each of which is a mention of named entity.
Here $P_s$ and $P_e$ are the start and end positions of a named entity mention, $t$ is the type of the mention from a predefined category set. Another one considers NER as a sequence labeling task, where each token is assigned to a special label (e.g. B-PER, I-PER, O). Figure \ref{fig:what is arabic ner} shows an example that an Arabic NER model recognizes three named entities from the given Arabic text. \textbf{Different from English or Chinese NER, the complexities of Arabic often makes the Arabic NER task extremely difficult. The most intuitive concern is the various form including CA, MSA and DA. For a simple example, the word "telephone" borrowed from English in MSA is "هاتف" (hātif) and the word might be "تلفون" (telfoon) in DA, while in CA , it does not have a term for "telephone" because the concept did not exist during that time. Besides, other challenges of Arabic NER will be the Obstacles to the development of this task, they will be detailed described in the next subsection.}


\subsection{The Challenges of Arabic NER}
NER is especially challenging when it comes to Arabic because of its particularities and unique nature. The main characteristics of Arabic that pose non-trivial challenges for NER tasks are as follows: 
\begin{itemize}
\item \textbf{No Capitalization}: 
Capitalization is a very distinguishing orthographic feature, such as proper names and abbreviations, which helps NER systems accurately recognize specific types of entities. Unlike English, where a named entity usually begins with a capital letter, capitalization is not a feature of the Arabic words. Consequently, only relying on looking up the items in the lexicon of proper nouns is not an appropriate solution to this problem\cite{algahtani2012arabic}.

\item \textbf{The Agglutinative Nature}: Arabic has a high agglutinative nature in which a word may consist of prefixes, lemma, and suffixes in different combinations, and that leads to a very complicated morphology\cite{abdelrahman2010integrated}. Meanwhile, named entities in Arabic are often associated with some other words, such as prepositions (e.g. for/to, as and by/with) or conjunctions (e.g. and)\cite{shaalan2014survey}. \textbf{For example, the prepositions "بـ" (bi, \textit{by/with}) in “بالقلم ” (\textit{with the pen}) and "بالسيارة " (\textit{by car}) will make the NER system confused. Also, the analysis of the fragment "القاهرة والإسكندرية" (\textit{Cairo and Alexander}) that contains a conjunctions "و" yields "الإسكندرية" (\textit{Alexander}) as a location name.} A common treatment is to obtain the text segmentation separated by a space character\cite{benajiba2007anersys2}.
% such as the word xx consists of the named entity xx and a conjunction xx, we would separate it by a space character to xx.

\item \textbf{Spelling Variants}: In Arabic, the word may be spelled differently and still refers to the same word with the same meaning, creating a many-to-one ambiguity, which is also called transcriptional ambiguity\cite{shaalan2007person}. \textbf{For instance, the word "مكتبة" (\textit{library}) can be spelled with diacritics as "مَكْتَبَة" or "مَكْتَبَه" and the word "مدرسة" (\textit{school}) can be written as "مَدْرَسَة" or "مَدْرَسَه" with the diacritics.}
% For example, there are some variants such as xx, xx, xx and xx when translating the named entity \textit{the city of Washington} from English to Arabic. 
To tackle this problem, researchers may normalize each variant to a unified form by a mechanism such as string distance calculation \cite{steinberger2012survey}.

\item \textbf{No Short Vowels}: Short vowels, or diacritics, are needed for pronunciation and disambiguation. However, most modern Arabic texts do not include diacritics. Therefore, one word form in Arabic may refer to two or more different words or meanings according to the context they appear, leading to a one-to-many ambiguity, which is easy to understand for a native Arabic speaker, but not for an Arabic NER system\cite{alkharashi2009person}. \textbf{For example, the word "جمال" can mean either "camel" in "ركبتُ الجمل لأول مرة في صحراء مصر" (\textit{I rode a camel for the first time in the Egyptian desert}) or "beauty" in "أعجبتني جمال الطبيعة في هذه المنطقة" (\textit{I was impressed by the beauty of nature in this region}) depending on the context in which it is used.} Short vowels are very important because different diacritics represent different meanings, which could help to disambiguate the structure and lexical types of Arabic entities. 
For a long time, these ambiguities caused by short vowels can only be solved by using contextual information and some knowledge of the language\cite{benajiba2009arabic}. Recently, with the introduction of the Arabic pre-trained models (e.g. AraBERT \cite{antoun2020arabert} and AraELECTRA \cite{antoun2021araelectra191}), the challenge caused by diacritics is further alleviated.

% \item \textbf{Different usage of Arabic}: 
% Distinguished from languages such as English and Chinese, different usages of Arabic have significant impacts on named entity recognition. Arabic can be commonly classified into three categories: Classical Arabic (CA), Modern Standard Arabic (MSA) and Dialects Arabic (DA) \cite{elgibali2005investigating}. 
% CA is the original Arabic language that has been used for over 1,500 years, and it is usually used in most Arabic religious texts. MSA is one of the official languages of the United Nations and widely used in today’s Arabic newspapers, letters and formal meetings, which is also be focused by researchers. DA is the spoken Arabic used in informal daily communication.
% For this reason, it is significant to confirm the difference between various uses of the Arabic language.


\item \textbf{Lacking Linguistic Resources}: 
Adequate data resources, including annotated corpus and high-quality lexicons/gazetteers, are critical to building a strong NER system. However, unlike the languages such as English and Chinese that have large-scaled tagged corpus, \textbf{there is a limitation in the number of available Arabic linguistic resources for Arabic NER due to the absence of annotations \cite{oudah2012pipeline}}. Even so, a few Arabic corpora have been created and publicly available for research purposes, we will introduce more details of these Arabic resources in the section 2.3.

\end{itemize}


\begin{figure*}[tb]
\centering
% \includegraphics[scale=0.6]{Figures/Arabic_NER_taxonomy.pdf}
\includegraphics[scale=0.7]{Figures/paradigms3.pdf}
\caption{The taxonomy of Arabic NER methods based on different methods. The rule-based method and machine learning method will be introduced in Sections 3.1 and 3.2. The methods of deep learning and pre-trained language model for Arabic NER will be described in Sections 3.3 and 3.4. In deep learning methods, we present the development of Arabic NER from three perspectives, including \text{input representations, context encoder, and label decoder}. In the pre-trained language model, we illustrate the Arabic NER methods according to their architectures and data collection scope.}
\label{fig:aner_deep_learning}
% \vspace{-4mm}
\end{figure*}


\subsection{Current Resources for Arabic NER}

In this section, we summarize some widely-used datasets and popular tools for Arabic NER. As shown in Table 2, most datasets are mainly developed by annotating news articles with a small number of entity types. \textbf{In consideration of the fact that certain Arabic NER corpora are exclusively accessible to individuals with paid license agreements, e.g., ACE 2003. It is difficult for researchers to access them as they are not free. Here we describe three representative datasets as below:} 
% As most works of Arabic NER report their results on ANER and AQMAR, here we also give a short description of these two datasets.
% As most works of Arabic NER report their results on ANER, here we also give a short description of this dataset.

ANERcorp\cite{benajiba2007anersys} consists of 316 articles from 11 diverse sources to acquire a generalized corpus and \text{is composed of a training set and a test set}. It contains 150,286 tokens. In addition to the traditional entities such as organization, location, and person, ANERcorp introduces the miscellaneous type to suggest a single class for entities that do not belong to any of the other classes. 
\textbf{It is worth noting that this dataset was split into many different configurations over the years which made it hard to compare fairly across papers and systems \cite{abdul2010simplified,zaghouani2012renar,morsi2013studying}}. In 2020, a group of researchers from CAMeL Lab met with the creator of the corpus to consult with him and collectively agree on an exact split, and accepted minor corrections from the original dataset. Thus, a new version is ANERcorp \footnote{https://camel.abudhabi.nyu.edu/anercorp/} is released and we suggest using this split as a standard dataset for evaluating NER performance in Arabic. 
% Different from the previous version, this new version does not have a development set. 
In this new version of the dataset, 
the sentences containing the first 5/6 of the words go to train and the rest go to test. The train split has 125,102 words and the test split has 25,008 words. 

\textbf{AQMAR\cite{mohit2012recall} is a small NER dataset based on Arabic Wikipedia which contains about 3,000 sentences. The creators picked 31 articles from history, technology, science, and sports areas that are suitable on the basis of length, cross-lingual linkages, and subjective judgments of quality. Compared with news text, the categories of Wikipedia articles are much more diverse. Accordingly, the traditional person, location and organization classes may not be suitable. And the appropriate entity classes can be quite different by domain. So AQMAR especially designs the custom entity categories for certain domains besides the classic ones.}

\textbf{CANERCorpus\cite{salah2018building} is proposed to support the studies of Classical Arabic  which is the official language of Quran and Hadith. Based on Islamic topics, the corpus contains more than 7000 Hadiths which covers all aspects of Prophet Muhammad's life and offers proper guidance to Islam. The named entity classes are especially designed for Islamic topics as well which covers Allah, Prophet, etc., which has not been handled before. Three experts with more than 5 years of experience in the field of computational linguistics completed the annotation. This work contributes a lot to the development of Classical Arabic.}

\textbf{Among these Arabic NER datasets, ANERcorp is the first to publish and followed by the most work, which represents the traditional Arabic NER. Besides the classic entity classes, ANER further incorporates domain entities in fields of history, technology, science and sports, which enables the studies of domain specific named entity recognition. However, compared with ANERcorp, it is much smaller. Before the CANERCorpus, there is no dataset for Classical Arabic. This dataset concentrates on the CA and annotates on large-scale standard Islamic corpus. Although the entity categories are also abundant, it is not so balanced. The propotion of some categories is even lower than 1\%.}

Besides the dataset, here we also introduce some commonly used Arabic NLP tools which contribute to Arabic NER processing. 
\textbf{Different from the end-to-end neural network Arabic NER models that directly take the Arabic tokens as input and output the NER labels, in the traditional feature-based era, there are some important preprocess steps for Arabic NER, such as tokenization and part-of-speech tagging.}
MADAMIRA\cite{pasha2014madamira} \footnote{https://camel.abudhabi.nyu.edu/madamira/} provides \textbf{an online web demo for} morphological analysis and disambiguation of Arabic. It is designed to deal with basic tasks which are often the first or intermediate steps of a complex system, including diacritization, lemmatization, morphological disambiguation, part-of-speech tagging, stemming, glossing, and tokenization. The input text is converted into the Buckwalter representations and passed to the morphological analysis. Then the SVM extracts closed-class features while the language models acquire open-class features. The ranking component scores the analysis list of each word, which is subsequently passed to the tokenization component. Both the base phase chunking component and named entity recognizer take SVM to process the analyses and tokenizations.
\textbf{As shown in MADAMIRA\cite{pasha2014madamira}, the Arabic NER component directly benefits from the outputs of previous components.}


\textbf{Word segmentation is a key preprocess step in Arabic NER. 
However, most segmenters focus on Modern Standard Arabic, and tend to perform poorly when dealing with Arabic text that contains dialectal vocabulary and grammar.
To process the dialectal Arabic text, Monroe et al. \cite{monroe-etal-2014-word} propose the Stanford Arabic segmenter that achieves 95.1\% F1 score on the Egyptian Arabic corpus.}
The Stanford Arabic segmenter \footnote{https://nlp.stanford.edu/projects/arabic.shtml} is an extension of the character-level conditional random field model. This segmenter expands the regular label space to introduce two Arabic-specific orthographic rules. 
Domain adaptation methods are applied to segment informal and dialectal Arabic text.

Farasa\cite{abdelali-etal-2016-farasa} \footnote{https://farasa.qcri.org/} is a fast and accurate Arabic segmenter based on SVM which ranks possible segmentations of a word by adopting a variety of features and lexicons. Farasa supports segmentation, stemming, named entity recognition, part of speech tagging and diacritization. The experiments demonstrate that this tool performs much better on the information retrieval tasks than Stanford Arabic segmenter and MADAMIRA.

As most Arabic NLP tools suffer from a lack of flexibility, CAMeL\cite{obeid2020camel} \footnote{https://github.com/CAMeL-Lab/camel\_tools} is presented to solve the problem. It is implemented in Python 3 and provides a series of pre-processing steps, such as transliteration and orthographic normalization. As for the named entity recognition, CAMeL fine-tunes the AraBert and experiments show that this tool outperforms the CRF-based system. 
\textbf{In more detail, CAMeL achieves 83\% overall F1 score on the ANERcorp dataset, surpassing the CRF-based system by a margin of 4\% F1 score.
Especially in the Person category, CAMeL achieves a 14\% improvement in F1 score compared to the CRF-based model.}





\subsection{Arabic NER metrics}

The metrics we take for Arabic NER are either the exact-match ones or the relaxed-match ones. For exact-match metrics, we evaluate the approaches with precision, recall, and F-score. Both the boundaries and entity type must be correct if the predicted entity is regarded as accurate. The precision suggests the ability to extract correct entities while the recall measures the ability to find as many entities as possible. Accordingly, F-score represents the balance of presion and recall. However, the exact-match metrics are somewhat too strict. Some approaches are also evaluated using relaxed-match metrics. For example, MUC-6\cite{grishman-sundheim-1996-message} propose to evaluate the system through the entity type and ignore the boundaries as long as there is an overlap with ground truth boundaries. Since the relaxed-match metric is complicated and inconvenient to analyze the bad cases, they are still not widely used.



==> challenges.tex <==
%guyingjie 蓝色是自己写过的，红色是直接copy的
\subsection{Challenges}
\textcolor{red}{Though significant progress has been achieved in Arabic NER research in the last decade, the task remains challenging due to the following features of the Arabic language; opportunities for improved performance are still available.}
\subsubsection{Different usage of Arabic}
\textcolor{blue}{Distinguished from languages such as English and Chinese, different usages of Arabic have great impact on named entity recognition. For this reason, it is significant to confirm the difference between various uses of the Arabic language.
Arabic can be commonly classified into three categorizes: Classical Arabic, Modern Standard Arabic and Colloquial Arabic Dialects.}

\textcolor{red}{CA is the formal version that has been used continuously for over 1,500 years as the language of Islam, used by Muslims in their daily prayers. Most Arabic religious texts are written in CA. In this context, person name recognition is of particular interest in order to identify and verify the correctness of citations (Zaraket and Makhlouta 2012) (a sequence of hadith narrators referencing each other who provide narrations related to the Prophet Mohammed based on known truthful and untruthful relaters). The importance of verification is that the authenticity of a hadith needs to be established before his narration is used in jurisprudence, and this depends on the credibility of the narrators.
Furthermore, many historical Arabic manuscripts are handwritten in CA (or Arabic
calligraphy); when they are digitized and converted to text, Arabic NE will become
important.
MSA is the language of today’s Arabic newspapers, magazines, periodicals, letters, modern writers, and education，which is one of the six official languages of the United Nations used in meetings and official UN documents. 
Most Arabic NLP, including NER research projects, is focused on MSA. The main difference between MSA and CA lies in the vocabulary, including NEs, and the orthography of conventional written Arabic.
Colloquial Arabic is the spoken Arabic used by Arabs in their informal daily communication; it is not taught in schools due to its irregularity. Unlike the widespread use of MSA across all Arab countries, colloquial Arabic is a regional variant that differs not only among Arab countries, but also across regions in the same country. Written Colloquial Arabic is presently used mainly in social media communication. For comparison, a person name in either CA or MSA could be expressed in Arabic dialect by more than one form; for example, PXA®Ë@ YJ
.« (Abd Al-Kader) versus PXAm.Ì'@ YJ.«(Abd Al-Gader) or PXB@ YJ.« (Abd Al-Aader). Salloum and Habash (2012) presented a universal machine translation pre-processing approach that has the ability to produce MSA paraphrases of dialectal input. In this way, available MSA tools can also be used to process Colloquial Arabic text, as most of the Arabic NER systems are developed to support MSA.
}


\subsubsection{Lack of Writing characteristics}
Incluing Capitalization and Uniformity in Writing Styles

\textcolor{red}{Unlike languages like English that use the Latin script, where most NEs begin with
a capital letter, capitalization is not a distinguishing orthographic feature of Arabic script for recognizing NEs such as proper names, acronyms, and abbreviations (Farber et al. 2008). The ambiguity caused by the absence of this feature is further increased by the fact that most Arabic proper nouns (NEs) are indistinguishable from forms that are common nouns and adjectives (non-NEs). Thus, an approach relying only on looking up entries in proper noun dictionaries would not be an appropriate way to tackle this problem, as ambiguous tokens/words that fall in this category are more likely to be used as non-proper nouns in text (Algahtani 2011). For example, the Arabic proper name 	 ¬Qå@ (Ashraf) can be used in a sentence as a given name, an inflected verb (he-supervised), and a superlative (the-most-honorable) (Mesfar 2007). An NE is usually found in a context, namely, with trigger and cue words to the left and/or right of the NE. Therefore, it is common to resolve this type of ambiguity by analyzing the context surrounding the NE. However, this might require deeper analysis of the NE’s context. As an example, consider the nominal sentence èYm.®Ó, whose literal meaning might be the falling of his head in grandfather/Jeddah. The
correct analysis of the trigger constituent éÓ as a multiword expression
denoting place of birth leads to the recognition of the following noun as a
location name.}

\textcolor{red}{Arabic has a high level of transcriptional ambiguity: An NE can be transliterated in a multitude of ways (Shaalan and Raza 2007). This multiplicity arises from both differences among Arabic writers and ambiguous transcription schemes (Halpern 2009). The lack of standardization is significant and leads to many variants of the same word that are spelled differently but still correspond to the same word with the same meaning, creating a many-to-one, variants-to-well-formed, ambiguity. For example, transcribing (also known as “Arabizing”) an NE such as the city of Washington into Arabic NE produces variants such as xxxx. One reason for this is
that Arabic has more speech sounds than Western European languages, which can
ambiguously or erroneously lead to an NE having more variants. One solution is to
retain all versions of the name variants with a possibility of linking them together. Another solution is to normalize each occurrence of the variant to a canonical form (Pouliquen et al. 2005); this requires a mechanism (such as string distance calculation) for name variant matching between a name variant and its normalized representation (Refaat and Madkour 2009; Steinberger 2012).}



\subsubsection{Low Resoureces}

